NL2SQL-BUGs: A Benchmark for Detecting Semantic Errors in NL2SQL Translation

Natural Language to SQL (i.e., NL2SQL) translation is crucial for democratizing database access, but even state-of-the-art models frequently generate semantically incorrect SQL queries, hindering the widespread adoption of these techniques by database vendors. While existing NL2SQL benchmarks primarily focus on correct query translation, we argue that a benchmark dedicated to identifying common errors in NL2SQL translations is equally important, as accurately detecting these errors is a prerequisite for any subsequent correction-whether performed by humans or models. To address this gap, we propose NL2SQL-BUGs, the first benchmark dedicated to detecting and categorizing semantic errors in NL2SQL translation. NL2SQL-BUGs adopts a two-level taxonomy to systematically classify semantic errors, covering 9 main categories and 31 subcategories. The benchmark consists of 2,018 expert-annotated instances, each containing a natural language query, database schema, and SQL query, with detailed error annotations for semantically incorrect queries. Through comprehensive experiments, we demonstrate that current large language models exhibit significant limitations in semantic error detection, achieving an average detection accuracy of 75.16%. Specifically, our method successfully detected 106 errors (accounting for 6.91%) in BIRD, a widely-used NL2SQL dataset, which were previously undetected annotation errors. This highlights the importance of semantic error detection in NL2SQL systems. The benchmark is publicly available at https://nl2sql-bugs.github.io/.

==> tables/error_type_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\caption{The taxonomy of NL2SQL errors.}
\label{tab:nl2sql_error_taxonomy}
\resizebox{\textwidth}{!}{
\begin{tabular}{|ccl|c|c|c|c|}
\hline
% SQL Components MainType
\multicolumn{1}{|c|}{\textbf{MainType}} &
  \multicolumn{1}{c|}{\textbf{SubType}} &
  \multicolumn{1}{c|}{\textbf{Description}} &
  \textbf{RESDSQL} &
  \textbf{Codes} &
  \textbf{Chess} &
  \textbf{Total} \\ \hline
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Comparison Operator} &
  The comparison operator {[}O{]} in condition {[}C{]}may be wrong. &
  \cellcolor[HTML]{EAF5EF}4 &
  \cellcolor[HTML]{E5F3EB}5 &
  \cellcolor[HTML]{E7F4ED}4 &
  \cellcolor[HTML]{E8F4ED}\textbf{13} \\ \cline{2-7} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\textbf{Operator Errors}}} &
  \multicolumn{1}{c|}{Logical Operator} &
  The boolean operator {[}O{]} maybe wrong. &
  \cellcolor[HTML]{EFF7F3}3 &
  \cellcolor[HTML]{F3F9F7}2 &
  \cellcolor[HTML]{F7FAFB}1 &
  \cellcolor[HTML]{F3F9F7}\textbf{6} \\ \hline
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Table Mismatch} &
  The table {[}T{]} may be wrong. &
  \cellcolor[HTML]{F3F9F7}2 &
  \cellcolor[HTML]{EFF7F3}3 &
  \cellcolor[HTML]{EDF6F2}3 &
  \cellcolor[HTML]{F0F7F4}\textbf{8} \\ \cline{2-7} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Table Redundancy} &
  The table {[}T{]} may be unnecessary. &
  \cellcolor[HTML]{68C07F}32 &
  \cellcolor[HTML]{C9E8D3}11 &
  \cellcolor[HTML]{ADDCBB}15 &
  \cellcolor[HTML]{9FD7AF}\textbf{58} \\ \cline{2-7} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Table Missing} &
  The table {[}T{]} may be missing. &
  \cellcolor[HTML]{EFF7F3}3 &
  \cellcolor[HTML]{E1F1E7}6 &
  \cellcolor[HTML]{E2F2E9}5 &
  \cellcolor[HTML]{E6F3EC}\textbf{14} \\ \cline{2-7} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Join Condition} &
  %There is no direct foreign key between {[}A{]} and {[}A{]}. &
  The join condition between table [T] and table [T] is incorrect. &
  \cellcolor[HTML]{C5E6CF}12 &
  \cellcolor[HTML]{E5F3EB}5 &
  \cellcolor[HTML]{D8EEE0}7 &
  \cellcolor[HTML]{D6EDDE}\textbf{24} \\ \cline{2-7} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{\textbf{Table-Related}}} &
  \multicolumn{1}{c|}{Join Type} &
  {\color[HTML]{0E0E0E} The join type {[}K{]} (e.g., LEFT JOIN) is inconsistent with the NL   intent.} &
  \cellcolor[HTML]{F8FBFB}1 &
  \cellcolor[HTML]{F8FBFB}1 &
  \cellcolor[HTML]{F7FAFB}1 &
  \cellcolor[HTML]{F8FBFB}\textbf{3} \\ \hline
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Explicit Condition missing} &
  The condition {[}C{]} in natural language may be missing. &
  \cellcolor[HTML]{B2DEBF}16 &
  \cellcolor[HTML]{D3ECDB}9 &
  \cellcolor[HTML]{EDF6F2}3 &
  \cellcolor[HTML]{CFEAD9}\textbf{28} \\ \cline{2-7} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Explicit Condition mismatch} &
  The condition {[}C{]} may be wrong. &
  \cellcolor[HTML]{E1F1E7}6 &
  \cellcolor[HTML]{D3ECDB}9 &
  \cellcolor[HTML]{C2E5CD}11 &
  \cellcolor[HTML]{D3ECDB}\textbf{26} \\ \cline{2-7} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Explicit Condition redundancy} &
  The condition {[}C{]} which not mentenditon in NL. &
  \cellcolor[HTML]{EAF5EF}4 &
  \cellcolor[HTML]{FCFCFF}0 &
  \cellcolor[HTML]{E2F2E9}5 &
  \cellcolor[HTML]{EEF7F3}\textbf{9} \\ \cline{2-7} 
\multicolumn{1}{|c|}{\multirow{-4}{*}{\textbf{Condition-Related}}} &
  \multicolumn{1}{c|}{Implicit Condition missing} &
  The query fails to include implicit conditions {[}C{]}(e.g., IS   NOT NULL). &
  \cellcolor[HTML]{D7EDDF}8 &
  \cellcolor[HTML]{C0E4CB}13 &
  \cellcolor[HTML]{C2E5CD}11 &
  \cellcolor[HTML]{C9E8D3}\textbf{32} \\ \hline
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Subquery missing} &
  The subquery {[}Q{]} missing. &
  \cellcolor[HTML]{E1F1E7}6 &
  \cellcolor[HTML]{E1F1E7}6 &
  \cellcolor[HTML]{E2F2E9}5 &
  \cellcolor[HTML]{E1F1E8}\textbf{17} \\ \cline{2-7} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Subquery redundancy} &
  The subquery {[}Q{]} redundancy. &
  \cellcolor[HTML]{FCFCFF}0 &
  \cellcolor[HTML]{FCFCFF}0 &
  \cellcolor[HTML]{FCFCFF}0 &
  \cellcolor[HTML]{FCFCFF}\textbf{0} \\ \cline{2-7} 
\multicolumn{1}{|c|}{\multirow{-3}{*}{\textbf{Subquery-Related}}} &
  \multicolumn{1}{c|}{Subquery mismatch} &
  The subquery {[}Q{]} mismatch. &
  \cellcolor[HTML]{FCFCFF}0 &
  \cellcolor[HTML]{FCFCFF}0 &
  \cellcolor[HTML]{F7FAFB}1 &
  \cellcolor[HTML]{FBFCFE}\textbf{1} \\ \hline
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Attribute Mismatch} &
  The attribute {[}A{]} may be wrong. &
  \cellcolor[HTML]{63BE7B}33 &
  \cellcolor[HTML]{63BE7B}33 &
  \cellcolor[HTML]{63BE7B}29 &
  \cellcolor[HTML]{63BE7B}\textbf{95} \\ \cline{2-7} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Attribute Redundancy} &
  The attribute {[}A{]} may not be mentioned in the natural   language. &
  \cellcolor[HTML]{E5F3EB}5 &
  \cellcolor[HTML]{E1F1E7}6 &
  \cellcolor[HTML]{D8EEE0}7 &
  \cellcolor[HTML]{E0F1E6}\textbf{18} \\ \cline{2-7} 
\multicolumn{1}{|c|}{\multirow{-3}{*}{\textbf{Attribute-Related}}} &
  \multicolumn{1}{c|}{Attribute Missing} &
  The attribute {[}A{]} may be missing. &
  \cellcolor[HTML]{F3F9F7}2 &
  \cellcolor[HTML]{E1F1E7}6 &
  \cellcolor[HTML]{E7F4ED}4 &
  \cellcolor[HTML]{E9F5EF}\textbf{12} \\ \hline
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Incorrect values} &
  The value {[}V{]} in condition {[}C{]} maybe wrong. &
  \cellcolor[HTML]{76C68B}29 &
  \cellcolor[HTML]{76C68B}29 &
  \cellcolor[HTML]{6EC385}27 &
  \cellcolor[HTML]{74C589}\textbf{85} \\ \cline{2-7} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\textbf{Value-Related}}} &
  \multicolumn{1}{c|}{Data format} &
  The data format of value {[}V{]} in attribute  {[}A{]} maybe wrong. &
  \cellcolor[HTML]{F8FBFB}1 &
  \cellcolor[HTML]{F3F9F7}2 &
  \cellcolor[HTML]{F7FAFB}1 &
  \cellcolor[HTML]{F6FAFA}\textbf{4} \\ \hline
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Aggregate Functions} &
  The usage of aggregate functions {[}F{]} (e.g., SUM, AVG) is   incorrect. &
  \cellcolor[HTML]{EAF5EF}4 &
  \cellcolor[HTML]{EAF5EF}4 &
  \cellcolor[HTML]{E2F2E9}5 &
  \cellcolor[HTML]{E8F4ED}\textbf{13} \\ \cline{2-7} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Window Functions} &
  The usage of window functions {[}F{]} (e.g., OVER) is incorrect. &
  \cellcolor[HTML]{F3F9F7}2 &
  \cellcolor[HTML]{F3F9F7}2 &
  \cellcolor[HTML]{F2F8F6}2 &
  \cellcolor[HTML]{F3F9F7}\textbf{6} \\ \cline{2-7} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Date/Time Functions} &
  The usage of date/time functions {[}F{]} (e.g., STRFTIME) is incorrect. &
  \cellcolor[HTML]{FCFCFF}0 &
  \cellcolor[HTML]{FCFCFF}0 &
  \cellcolor[HTML]{FCFCFF}0 &
  \cellcolor[HTML]{FCFCFF}\textbf{0} \\ \cline{2-7} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Conversion Functions} &
  The usage of conversion functions {[}F{]} (e.g., CAST) is   incorrect. &
  \cellcolor[HTML]{F8FBFB}1 &
  \cellcolor[HTML]{F8FBFB}1 &
  \cellcolor[HTML]{FCFCFF}0 &
  \cellcolor[HTML]{F9FBFD}\textbf{2} \\ \cline{2-7} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Math Functions} &
  The usage of math functions {[}F{]} (e.g., ROUND) is incorrect. &
  \cellcolor[HTML]{DCEFE3}7 &
  \cellcolor[HTML]{D7EDDF}8 &
  \cellcolor[HTML]{D2EBDB}8 &
  \cellcolor[HTML]{D7EDE0}\textbf{23} \\ \cline{2-7} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{String Functions} &
  The usage of string functions {[}F{]} (e.g., SUBSTR) is incorrect. &
  \cellcolor[HTML]{F8FBFB}1 &
  \cellcolor[HTML]{F8FBFB}1 &
  \cellcolor[HTML]{FCFCFF}0 &
  \cellcolor[HTML]{F9FBFD}\textbf{2} \\ \cline{2-7} 
\multicolumn{1}{|c|}{\multirow{-7}{*}{\textbf{Function-Related}}} &
  \multicolumn{1}{c|}{Conditional Functions} &
  The usage of conditional functions {[}F{]} (e.g., IIF)  is incorrect. &
  \cellcolor[HTML]{CEEAD7}10 &
  \cellcolor[HTML]{D3ECDB}9 &
  \cellcolor[HTML]{C8E7D2}10 &
  \cellcolor[HTML]{CEEAD7}\textbf{29} \\ \hline
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Clause Missing} &
  Clause {[}K{]} Missing &
  \cellcolor[HTML]{D7EDDF}8 &
  \cellcolor[HTML]{D3ECDB}9 &
  \cellcolor[HTML]{D2EBDB}8 &
  \cellcolor[HTML]{D4ECDD}\textbf{25} \\ \cline{2-7} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Clause Redundancy} &
  Clause {[}K{]} Redundancy &
  \cellcolor[HTML]{EAF5EF}4 &
  \cellcolor[HTML]{F3F9F7}2 &
  \cellcolor[HTML]{DDF0E4}6 &
  \cellcolor[HTML]{E9F5EF}\textbf{12} \\ \cline{2-7} 
\multicolumn{1}{|c|}{\multirow{-3}{*}{\textbf{Clause-Related}}} &
  \multicolumn{1}{c|}{LIMIT Clause Offset} &
  LIMIT Clause Offset {[}V{]} &
  \cellcolor[HTML]{F8FBFB}1 &
  \cellcolor[HTML]{F3F9F7}2 &
  \cellcolor[HTML]{EDF6F2}3 &
  \cellcolor[HTML]{F3F9F7}\textbf{6} \\ \hline
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{DISTINCT} &
  DISTINCT &
  \cellcolor[HTML]{A4D9B3}19 &
  \cellcolor[HTML]{A0D7AF}20 &
  \cellcolor[HTML]{8ED0A0}21 &
  \cellcolor[HTML]{9CD5AC}\textbf{60} \\ \cline{2-7} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Other} &
  Other(orderby vs. limit 1 bird data cause) &
  \cellcolor[HTML]{D7EDDF}8 &
  \cellcolor[HTML]{EFF7F3}3 &
  \cellcolor[HTML]{EDF6F2}3 &
  \cellcolor[HTML]{E6F3EC}\textbf{14} \\ \cline{2-7} 
\multicolumn{1}{|c|}{\multirow{-3}{*}{\textbf{Other}}} &
  \multicolumn{1}{c|}{Syntax} &
  Syntax &
  \cellcolor[HTML]{9BD5AB}21 &
  \cellcolor[HTML]{F3F9F7}2 &
  \cellcolor[HTML]{F7FAFB}1 &
  \cellcolor[HTML]{D6EDDE}\textbf{24} \\ \hline
\multicolumn{3}{|c|}{\textbf{Total}} &
  \textbf{253} &
  \textbf{209} &
  \textbf{207} &
  \textbf{669} \\ \hline
\end{tabular}}
\end{table*}
